Reinforcement Learning with Large Action Spaces for Neural Machine Translation

Applying Reinforcement learning (RL) following maximum likelihood estimation (MLE) pre-training is a versatile method for enhancing neural machine translation (NMT) performance. However, recent work has argued that the gains produced by RL for NMT are mostly due to promoting tokens that have already received a fairly high probability in pre-training. We hypothesize that the large action space is a main obstacle to RL's effectiveness in MT, and conduct two sets of experiments that lend support to our hypothesis. First, we find that reducing the size of the vocabulary improves RL's effectiveness. Second, we find that effectively reducing the dimension of the action space without changing the vocabulary also yields notable improvement as evaluated by BLEU, semantic similarity, and human evaluation. Indeed, by initializing the network's final fully connected layer (that maps the network's internal dimension to the vocabulary dimension), with a layer that generalizes over similar actions, we obtain a substantial improvement in RL performance: 1.5 BLEU points on average.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> table.tex <==
\begin{table}[tb!]
\centering
\begin{subtable}{0.5\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{cos_dis_mod.png} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lllll@{}}
\toprule
MODEL           & De-En & Cs-En & Ru-En & Tr-En \\ \midrule
MLE             & 22.38 & 15.81 & 17.31 & 12.60 \\
+RL             & 23.19 & 15.81 & 17.31 & 12.66 \\
% \hline
\midrule

% \hline
% \hline
+RL+FREEZE      & 23.14 & 16.04 & 17.78 & 13.18 \\
% \midrule
+BERT           & 23.46 & 16.59 & 18.14 & 14.15 \\
+BERT+RL       & 24.44 & 17.04 & \textbf{18.68} & 14.37 \\
+BERT+RL+FREEZE & \textbf{24.71} & \textbf{17.37} & 18.30 & \textbf{14.55} \\ \bottomrule
\end{tabular}}
    \caption{BLEU (SacreBLEU) scores}
    \label{tab:my_label_blue}
\end{subtable}
\begin{subtable}{0.5\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{cos_dis_bert.png}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lllll@{}}
\toprule
MODEL           & De-En & Cs-En & Ru-En & Tr-En \\ \midrule
MLE             & 70.03 & 63.29 & 66.17 & 59.68 \\
+RL             & 71.17 & 63.29 & 66.17 & 59.99 \\
% \hline
\midrule

% \hline
% \hline
+RL+FREEZE      & 71.03 & 64.29 & 66.66 & 60.52 \\
% \midrule
+BERT          & 71.56 & 64.26 & 66.70 & 61.75 \\
+BERT+RL       & 72.44 & 65.80 & \textbf{67.94} & \textbf{63.59} \\
+BERT+RL+FREEZE & \textbf{72.81} & \textbf{66.44} & 67.66 & \textbf{63.59} \\ \bottomrule
\end{tabular}}
    \caption{SIM scores}
    \label{tab:my_label_sim}
\end{subtable}
\caption{BLEU/SIM scores on translating four languages to English.
The upper block, in each table, shows the baseline scores of training only with MLE, and with MLE followed by RL. RL presents modest improvement (if any) over only using MLE.
+RL+FREEZE shows some improvement due to freezing the target embeddings.
The lower three rows show results when using BERT's target embeddings (informative initialization).
%RL is more effective in this setting (the difference between +RL+BERT and +BERT is greater than the difference between +RL and MLE). 
Additional benefit is seen from freezing (+RL+BERT+FREEZE). \vspace{-.5cm}}
\label{tab:table-BERT-results}
\end{table}


% % figure 2:
% \begin{table}
% \begin{subtable}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}lllll@{}}
% \toprule
% MODEL           & De-En & Cs-En & Ru-En & Rr-En \\ \midrule
% MLE             & 22.38 & 15.81 & 17.31 & 12.60 \\
% +RL             & 23.19 & 15.81 & 17.31 & 12.66 \\
% % \hline
% \midrule

% % \hline
% % \hline
% +RL+FREEZE      & 23.14 & 16.04 & 17.78 & 13.18 \\
% % \midrule
% +BERT           & 23.46 & 16.59 & 18.14 & 14.15 \\
% +BERT+RL       & 24.44 & 17.04 & \textbf{18.68} & 14.37 \\
% +BERT+RL+FREEZE & \textbf{24.71} & \textbf{17.37} & 18.30 & \textbf{14.55} \\ \bottomrule
% \end{tabular}
% }
% \label{tab:table1_a}
% \end{subtable}

% \centering
% \begin{subtable}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}lllll@{}}
% \toprule
% MODEL           & de-en & cs-en & ru-en & tr-en \\ \midrule
% MLE             & 70.03 & 63.29 & 66.17 & 59.68 \\
% +RL             & 71.17 & 63.29 & 66.17 & 59.99 \\
% % \hline
% \midrule

% % \hline
% % \hline
% +RL+FREEZE      & 71.03 & 64.29 & 66.66 & 60.52 \\
% % \midrule
% +BERT          & 71.56 & 64.26 & 66.70 & 61.75 \\
% +BERT+RL       & 72.44 & 65.80 & \textbf{67.94} & \textbf{63.59} \\
% +BERT+RL+FREEZE & \textbf{72.81} & \textbf{66.44} & 67.66 & \textbf{63.59} \\ \bottomrule
% \end{tabular}
% }\caption{\label{tab:table-BERT-results}BLEU (SacreBLEU) and SIM scores (up/down) on translating four languages to English.
% The upper block shows the baseline scores of training only with MLE, and with MLE followed by RL. RL presents modest improvement (if any) over only using MLE.
% +RL+FREEZE shows some improvement due to freezing the target embeddings.
% The lower three rows show results when using BERT's target embeddings (informative initialization).
% %RL is more effective in this setting (the difference between +RL+BERT and +BERT is greater than the difference between +RL and MLE). 
% Additional benefit is seen from freezing (+RL+BERT+FREEZE). \vspace{-.5cm}}
% \label{tab:table1}
% \end{subtable}
% \end{table}





% % % \documentclass{article}
% % % \usepackage{subcaption,booktabs}
% % \begin{document}

% % \begin{table}   
% % %\centering  <--- not needed!
% % \begin{subtable}{.5\textwidth}
% % \centering
% %   % dummy 'tabular' env.
% %   \begin{tabular}{lll}
% %   \toprule
% %   aaa bbb ccc\\
% %   \bottomrule
% %   \end{tabular}
% % \caption{Phase 1}
% % \end{subtable}% <--- new
% % \begin{subtable}{.5\textwidth}
% % \centering 
% %   % dummy 'tabular' env.
% %   \begin{tabular}{lll}
% %   \toprule
% %   xxx yyy zzz\\
% %   \bottomrule
% %   \end{tabular}
% % \caption{Phase 2}
% % \end{subtable}
% % \caption{aaaaaaa} \label{tab:EmMaxPE_bar_X}
% % \end{table}
% % \end{document}
